Maser Activity of Organic Molecules toward Sgr B2(N)

At centimeter wavelengths, single-dish observations have suggested that the Sagittarius (Sgr) B2 molecular cloud at the Galactic Center hosts weak maser emission from several organic molecules, including CH$_2$NH, HNCNH, and HCOOCH$_3$. However, the lack of spatial distribution information of these new maser species has prevented us from assessing the excitation conditions of the maser emission as well as their pumping mechanisms. Here, we present a mapping study toward Sgr B2 North (N) to locate the region where the complex maser emission originates. We report the first detection of the Class I methanol (CH$_3$OH) maser at 84 GHz and the first interferometric map of the methanimine (CH$_2$NH) maser at 5.29 GHz toward this region. In addition, we present a tool for modeling and fitting the unsaturated molecular maser signals with non-LTE radiative transfer models and Bayesian analysis using the Markov-Chain Monte Carlo approach. These enable us to quantitatively assess the observed spectral profiles. The results suggest a two-chain-clump model for explaining the intense CH$_3$OH Class I maser emission toward a region with low continuum background radiation. By comparing the spatial origin and extent of maser emission from several molecular species, we find that the 5.29 GHz CH$_2$NH maser has a close spatial relationship with the 84 GHz CH$_3$OH Class I masers. This relationship serves as observational evidence to suggest a similar collisional pumping mechanism for these maser transitions.

==> coll.tex <==


For Section 4.1
-----------------

The molecular data file for $E$-type \ce{CH3OH} was taken from the
Excitation of Molecules and Atoms for Astrophysics (EMAA)
database \footnote{\footnotesize{https://emaa.osug.fr}}, with
spectroscopy from the Cologne Database for Molecular Spectroscopy
(CDMS)
catalog\footnote{\footnotesize{https://www.astro.uni-koeln.de/cdms/catalog}} \citep{2005JMoSt.742..215M}
and collision rate coefficients reported
by \citet{2010MNRAS.406...95R} for the rotational excitation
of \ce{CH3OH} by para- and ortho-H$_2$ (hereafter p-H$-2$ and
o-H$_2$). The calculations of \citet{2010MNRAS.406...95R} were
performed for rotational transitions within the three first torsional
states of methanol, $\nu=0, 1, 2$, with a methanol basis including
rotational states $j_1\leq 15$ for p-H$_2(j_2=0)$ and $j_1\leq 9$ for
o-H$_2(j_2=1)$ (where $j_1$ and $j_2$ are the rotational quantum
numbers). The coupled-states approximation was used to generate rate
coefficients at temperatures $10 \leq T_k \leq 200$~K. Because
torsionally inelastic transitions were not considered
by \citet{2010MNRAS.406...95R}, the EMAA dataset for $E$-CH$_3$OH
includes rotational transitions within the ground torsional state
($\nu=0$) only. The first excited state ($\nu=1$) of $E$-\ce{CH3OH}
opening at 204.2~cm$^{-1}$, the highest level of $E$-\ce{CH3OH}
included in the EMAA dataset is the rotational state 9(-6) ($j_1=9,
K=-6$) with an energy of 203.9~cm$^{-1}$.


For Section 4.2
----------------

A first set of collisional data for CH$_2$NH + p-H$_2(j_2=0)$ was
published by
\citet{2018JPCL....9.3199F} for applications to cold gas.  The calculations
of \citet{2018JPCL....9.3199F} were performed for rotational
transitions among the first 15 rotational levels of \ce{CH2NH},
i.e. up to the state 2(2, 0) ($j_1=2, K_a=2, K_c=0$) with an energy of
28.3~cm$^{-1}$. The full close-coupling method was used to generate
rate coefficients at temperatures $5 \leq T_k \leq 30$~K and
hyperfine-resolved rate coefficients were derived from the rotational
rate coefficients using the statistical approximation,
see \citet{2018JPCL....9.3199F} for full details. In this work, we
have extended the calculations of \citet{2018JPCL....9.3199F} to
higher levels and temperatures and we have thus considered
o-H$_2(j_2=1)$ as a second collider. Because close-coupling
calculations are computationally very demanding when the temperature
increases, we had recourse to the coupled-state approximation. As
in \citet{2018JPCL....9.3199F}, all calculations were performed with
the OpenMP extension\footenote{See
http://ipag.osug.fr/$\sim$faurea/molscat/index.html} of the version 14
of the \texttt{MOLSCAT} code \citep{molscat}, using the same
propagation parameters and rotational basis for CH$_2$NH ($j_1\leq
12$) and para-H$_2$ ($j_2=0, 2$). The basis for ortho-H$_2$ was
restricted to $j_2=1$ and the \texttt{MOLSCAT} parameter \texttt{EMAX}
(used to limit basis functions to CH$_2$NH plus H$_2$ energies less
than
\texttt{EMAX}) was set to 1200~cm$^{-1}$ for p-H$_2$ and
1318.64~cm$^{-1}$ for o-H$_2$. The coupled-state calculations were
performed for total energies between 2 and 800 cm$^{-1}$ for
para-H$_2$ and between 120 and 918~cm$^{-1}$ for ortho-H$_2$. Rate
coefficients were obtained for all rotational transitions among the
first 49 levels, i.e. up to the state 8(2, 6) at 99.5~cm$^{-1}$, and
for kinetic temperatures in the range 10-150~K. Hyperfine-resolved
rate coefficients were derived using the statistical approximation, as
in \citet{2018JPCL....9.3199F}. Finally, the collisional dataset was combined with
the energy levels and radiative rates taken from the CDMS catalog
\citep{2005JMoSt.742..215M} in order to provide an EMAA-formatted datafile.


@MISC{molscat, author = {{Hutson}, J.~M. and {Green}, S.}, title =
   "{MOLSCAT: MOLecular SCATtering}", keywords = {Software },
   howpublished = {Astrophysics Source Code Library}, year = 2012,
   month = jun, archivePrefix = "ascl", eprint = {1206.004}, adsurl =
   {http://adsabs.harvard.edu/abs/2012ascl.soft06004H}, adsnote =
   {Provided by the SAO/NASA Astrophysics Data System} }


